Decentralized Equalization with Feedforward Architectures for Massive MU-MIMO

Linear data-detection algorithms that build on zero forcing (ZF) or linear minimum mean-square error (L-MMSE) equalization achieve near-optimal spectral efficiency in massive multi-user multiple-input multiple-output (MU-MIMO) systems. Such algorithms, however, typically rely on centralized processing at the base-station (BS) which results in (i) excessive interconnect and chip input/output (I/O) data rates and (ii) high computational complexity. Decentralized baseband processing (DBP) partitions the BS antenna array into independent clusters that are associated with separate radio-frequency circuitry and computing fabrics in order to overcome the limitations of centralized processing. In this paper, we investigate decentralized equalization with feedforward architectures that minimize the latency bottlenecks of existing DBP solutions. We propose two distinct architectures with different interconnect and I/O bandwidth requirements that fuse the local equalization results of each cluster in a feedforward network. For both architectures, we consider maximum ratio combining, ZF, L-MMSE, and a nonlinear equalization algorithm that relies on approximate message passing, and we analyze the associated post-equalization signal-to-noise-and-interference-ratio (SINR). We provide reference implementation results on a multi graphics processing unit (GPU) system which demonstrate that decentralized equalization with feedforward architectures enables throughputs in the Gb/s regime and incurs no or only a small performance loss compared to centralized solutions.

==> macros/delta_star.tex <==
% This file was created by matlab2tikz v0.4.7 running on MATLAB 8.1.
% Copyright (c) 2008--2014, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% Minimal pgfplots version: 1.3
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
\begin{tikzpicture}

\begin{axis}[%
width=5.16317052165354in,
height=3.59478807824803in,
scale only axis,
xmin=0.5,
xmax=1,
xlabel={$\sigma{}^\text{2}$},
xmajorgrids,
ymin=-0.1,
ymax=0.02,
ylabel={$\text{MSE }\Psi\text{(}\sigma{}^\text{2}\text{,}\delta\text{)}$},
ymajorgrids,
legend style={draw=black,fill=white,legend cell align=left},
scaled y ticks = false,
y tick label style={/pgf/number format/.cd, fixed, fixed zerofill,precision=2}
]
\addplot [color=blue,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.00847186823552865\\
0.51	-0.00601453905159377\\
0.52	-0.00370544732742462\\
0.53	-0.00154476341156906\\
0.54	0.000467627376738888\\
0.55	0.00233209087222286\\
0.56	0.00404921374335487\\
0.57	0.0056197763556024\\
0.58	0.0070447284855838\\
0.59	0.00832516758867108\\
0.6	0.00946231935404707\\
0.61	0.010457520309356\\
0.62	0.0113122022622594\\
0.63	0.0120278783886857\\
0.64	0.0126061307976336\\
0.65	0.0130485994203295\\
0.66	0.0133569720875105\\
0.67	0.0135329756729161\\
0.68	0.0135783681937844\\
0.69	0.0134949317705579\\
0.7	0.0132844663581388\\
0.71	0.0129487841701174\\
0.72	0.0124897047255125\\
0.73	0.0119090504547793\\
0.74	0.0112086428083547\\
0.75	0.0103902988167651\\
0.76	0.00945582805653367\\
0.77	0.0084070299807415\\
0.78	0.00724569157726995\\
0.79	0.00597358532146186\\
0.8	0.0045924673932799\\
0.81	0.003104076132037\\
0.82	0.00151013070445061\\
0.83	-0.000187670035805887\\
0.84	-0.00198764851672595\\
0.85	-0.0038881492624897\\
0.86	-0.00588753956984844\\
0.87	-0.00798421006078442\\
0.88	-0.0101765751244192\\
0.89	-0.0124630732598896\\
0.9	-0.0148421673307546\\
0.91	-0.0173123447404596\\
0.92	-0.0198721175374564\\
0.93	-0.0225200224577413\\
0.94	-0.0252546209118061\\
0.95	-0.0280744989223199\\
0.96	-0.0309782670182411\\
0.97	-0.0339645600904978\\
0.98	-0.037032037213876\\
0.99	-0.0401793814392991\\
1	-0.0434052995602611\\
};
\addlegendentry{$\delta\text{=0.48}$};

\addplot [color=black!50!green,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.0187120376472885\\
0.51	-0.0165142361546856\\
0.52	-0.0144615838414366\\
0.53	-0.0125542475071614\\
0.54	-0.0107921148602765\\
0.55	-0.00917482768761513\\
0.56	-0.00770181154296512\\
0.57	-0.00637230231847263\\
0.58	-0.00518537002453257\\
0.59	-0.00413994006942631\\
0.6	-0.00323481229916234\\
0.61	-0.00246867803042228\\
0.62	-0.00184013528487104\\
0.63	-0.00134770241107862\\
0.64	-0.00098983026065036\\
0.65	-0.000764913067593964\\
0.66	-0.000671298164312661\\
0.67	-0.000707294653602974\\
0.68	-0.000871181143586086\\
0.69	-0.00116121264132862\\
0.7	-0.0015756266909891\\
0.71	-0.00211264883342677\\
0.72	-0.00277049745626901\\
0.73	-0.0035473880963619\\
0.74	-0.00444153725015284\\
0.75	-0.00545116574191751\\
0.76	-0.00657450169464413\\
0.77	-0.00780978314385727\\
0.78	-0.00915526033058989\\
0.79	-0.0106091977060686\\
0.8	-0.0121698756774135\\
0.81	-0.0138355921207137\\
0.82	-0.0156046636852255\\
0.83	-0.01747542691006\\
0.84	-0.0194462391726276\\
0.85	-0.0215154794861878\\
0.86	-0.0236815491621433\\
0.87	-0.0259428723511849\\
0.88	-0.0282978964759938\\
0.89	-0.0307450925669753\\
0.9	-0.0332829555113638\\
0.91	-0.0359100042250333\\
0.92	-0.0386247817554261\\
0.93	-0.0414258553232051\\
0.94	-0.0443118163094768\\
0.95	-0.0472812801947716\\
0.96	-0.050332886455361\\
0.97	-0.0534652984219457\\
0.98	-0.0566772031052537\\
0.99	-0.0599673109926471\\
1	-0.0633343558194223\\
};
\addlegendentry{$\delta\text{=0.49}$};

\addplot [color=red,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.0285342409606091\\
0.51	-0.0265853741923451\\
0.52	-0.0247786943752848\\
0.53	-0.0231143649049744\\
0.54	-0.0215922757814954\\
0.55	-0.0202120761021536\\
0.56	-0.0189732031441291\\
0.57	-0.0178749083936059\\
0.58	-0.0169162808403585\\
0.59	-0.0160962678231115\\
0.6	-0.015413693680812\\
0.61	-0.0148672764379647\\
0.62	-0.0144556427280369\\
0.63	-0.0141773411373831\\
0.64	-0.0140308541328821\\
0.65	-0.0140146087192757\\
0.66	-0.0141269859568777\\
0.67	-0.0143663294565907\\
0.68	-0.0147309529569823\\
0.69	-0.0152191470772199\\
0.7	-0.0158291853299485\\
0.71	-0.0165593294694794\\
0.72	-0.0174078342428757\\
0.73	-0.0183729516045994\\
0.74	-0.0194529344491293\\
0.75	-0.0206460399104498\\
0.76	-0.0219505322723045\\
0.77	-0.0233646855286765\\
0.78	-0.0248867856299656\\
0.79	-0.0265151324467612\\
0.8	-0.0282480414799152\\
0.81	-0.03008384534274\\
0.82	-0.0320208950385883\\
0.83	-0.0340575610547527\\
0.84	-0.0361922342915535\\
0.85	-0.0384233268436126\\
0.86	-0.0407492726486302\\
0.87	-0.0431685280174872\\
0.88	-0.0456795720581163\\
0.89	-0.0482809070043839\\
0.9	-0.0509710584601116\\
0.91	-0.0537485755673797\\
0.92	-0.0566120311073562\\
0.93	-0.0595600215410989\\
0.94	-0.0625911669970385\\
0.95	-0.0657041112112049\\
0.96	-0.0688975214256599\\
0.97	-0.0721700882500693\\
0.98	-0.0755205254908607\\
0.99	-0.0789475699519808\\
1	-0.0824499812108627\\
};
\addlegendentry{$\delta\text{=0.50}$};

\end{axis}
\end{tikzpicture}%
